Binary Radiance Fields

In this paper, we propose \textit{binary radiance fields} (BiRF), a storage-efficient radiance field representation employing binary feature encoding that encodes local features using binary encoding parameters in a format of either $+1$ or $-1$. This binarization strategy lets us represent the feature grid with highly compact feature encoding and a dramatic reduction in storage size. Furthermore, our 2D-3D hybrid feature grid design enhances the compactness of feature encoding as the 3D grid includes main components while 2D grids capture details. In our experiments, binary radiance field representation successfully outperforms the reconstruction performance of state-of-the-art (SOTA) efficient radiance field models with lower storage allocation. In particular, our model achieves impressive results in static scene reconstruction, with a PSNR of 32.03 dB for Synthetic-NeRF scenes, 34.48 dB for Synthetic-NSVF scenes, 28.20 dB for Tanks and Temples scenes while only utilizing 0.5 MB of storage space, respectively. We hope the proposed binary radiance field representation will make radiance fields more accessible without a storage bottleneck.

==> figs/main/binary_encoding.tex <==
\begin{figure*}[!ht]
\begin{center}
\vspace{-4mm}
\includegraphics[width=0.9\linewidth]{assets/main/binary_encoding.pdf}
\end{center}
\vspace{-4mm}
\caption{Illustration of binary feature encoding.}
\label{fig:overall}
\end{figure*}

==> figs/main/sparsity.tex <==
\begin{figure*}[!ht]
\begin{center}
\vspace{-4mm}
\includegraphics[width=0.5\linewidth]{assets/main/sparsity.pdf}
\end{center}
\vspace{-4mm}
\caption{Visualization of an occupancy grid slice on the use of sparsity loss $\mathcal{L}_{\text{sparsity}}$.}
\label{fig:ablation_sparsity}
\end{figure*}

==> figs/rebuttal/ablation_binarization.tex <==
\begin{figure*}[!h]
\begin{center}
\vspace{-2mm}
\includegraphics[width=0.8\linewidth]{assets/rebuttal/ablation_quality_bfe.pdf}
\end{center}
\vspace{-2mm}
\caption{Ablation study on the binary feature encoding. Results are averaged over all scenes of the Synthetic-NeRF dataset, Synthetic-NSVF dataset, and Tanks and Temples dataset.}
\label{fig:ablation_binarization}
\end{figure*}

==> figs/rebuttal/convergence_comparison.tex <==
\begin{figure*}[!h]
\vspace{-2mm}
\begin{minipage}[b]{0.39\textwidth}
    \begin{center}
    \includegraphics[width=\linewidth]{assets/rebuttal/hashsize_extend.pdf}
    \end{center}
\vspace{-4mm}
\caption{Ablation study on the hash table size. Results are averaged over all scenes of the Synthetic-NeRF dataset.}
\label{fig:ablation_sparsity}
\end{minipage}\hfill
\begin{minipage}[b]{0.59\textwidth}
    \begin{center}
    \includegraphics[width=0.99\linewidth]{assets/rebuttal/convergence_comparison.pdf}
    \end{center}
\vspace{-4mm}
\caption{Evaluation of the reconstruction quality for the whole training time (up) and 1 min (bottom). ``Real-valued'' denotes a real-valued grid and ``binary'' denotes a binary grid.}
\label{fig:convergence_comparison}
\end{minipage}
\end{figure*}


==> figs/rebuttal/hash_collision.tex <==
\begin{figure*}[!h]
\vspace{-2mm}
\begin{minipage}[b]{0.34\textwidth}
    \begin{center}
    \includegraphics[width=0.9\linewidth]{assets/rebuttal/hash_collision.pdf}
    \end{center}
\vspace{-4mm}
\caption{Evaluation of hash collision frequencies based on different grid designs, 2D grid and 3D grid. $T$ denotes the size of the hash table. We set the maximum resolution to $1024$.}
\label{fig:hash_collision}
\end{minipage}\hfill
\begin{minipage}[b]{0.64\textwidth}
    \begin{center}
    \includegraphics[width=\linewidth]{assets/rebuttal/post_quant_qual.pdf}
    \end{center}
\vspace{-4mm}
\caption{Comparison of reconstruction quality according to the number of bits. ``Post-quant.'' denotes post-quantization.}
\label{fig:post_quant}
\end{minipage}
\end{figure*}

% \begin{figure*}[!ht]
% \begin{center}
% \vspace{-2mm}
% \includegraphics[width=0.65\linewidth]{assets/rebuttal/hash_collision.pdf}
% \end{center}
% \vspace{-2mm}
% \caption{Evaluation of hash collision frequencies based on different grid designs, 2D grid and 3D grid. $T$ denotes the size of the hash table. We set the maximum resolution to $1024$.}
% \label{fig:inference_time}
% \end{figure*}

==> figs/rebuttal/post_quantization.tex <==
% \begin{figure*}[!h]
% \vspace{-2mm}
% \begin{minipage}[b]{0.70\textwidth}
%     \begin{center}
%     \includegraphics[width=\linewidth]{assets/rebuttal/post_quant_qual.pdf}
%     \end{center}
% \vspace{-4mm}
% \caption{Ablation study on the hash table size. Results are averaged over all scenes of the Synthetic-NeRF dataset.}
% \label{fig:post_quant_qual}
% \end{minipage}\hfill
% \begin{minipage}[b]{0.30\textwidth}
%     \begin{center}
%     \includegraphics[width=0.95\linewidth]{assets/rebuttal/post_quantization.pdf}
%     \end{center}
% \vspace{-4mm}
% \caption{Comparison of reconstruction quality of binary feature grid and real-valued feature grid according to the time. We use Ours-F1 for this experiment.}
% \label{fig:post_quant}
% \end{minipage}
% \end{figure*}


\begin{figure*}[!h]
\begin{center}
\vspace{-2mm}
\includegraphics[width=0.9\linewidth]{assets/rebuttal/post_quant_qual.pdf}
\end{center}
\vspace{-2mm}
\caption{poste quant.}
\label{fig:inference_time}
\end{figure*}

==> tables/main/ablation_grid.tex <==
\begin{table}[!ht]
    \centering
    \resizebox{0.5\textwidth}{!}{
    \begin{tabular}{lccc}
        \toprule
        Design & \# Params & PSNR$\uparrow$ & SSIM$\uparrow$ \\
        \midrule
        Tri-plane (only 2D) & 13.7 M & 31.44 & 0.949 \\
        Voxel (only 3D) & 13.6 M & 32.35 & 0.958 \\
        Hybrid (2D + 3D) & 13.2 M & \textbf{32.64} & \textbf{0.959} \\
        \bottomrule
    \end{tabular}
    }
    \vspace{+2mm}
    \caption{Ablation evaluations on the feature grid design. Results are averaged over the all scenes of Synthetic-NeRF dataset. We highlight the best scores in \textbf{bold}.}
    \label{tab:ablation_grid}
\end{table}


% \begin{table}[!ht]
%     \centering
%     \resizebox{0.8\textwidth}{!}{
%     \begin{tabular}{lccccccc}
%         \toprule
%             \multirow{2}{*}{Method} & &
%             \multicolumn{2}{c}{Synthetic-NeRF} &
%             \multicolumn{2}{c}{Synthetic-NSVF} &
%             \multicolumn{2}{c}{Tanks \& Temples} \\
%             \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8}
%             & \# Params
%             % & Time (min)$\downarrow$
%             & PSNR$\uparrow$ & SSIM$\uparrow$ 
%             & PSNR$\uparrow$ & SSIM$\uparrow$ 
%             & PSNR$\uparrow$ & SSIM$\uparrow$   \\
%         \midrule
%         Tri-plane (only 2D) & 13.7 M
%         & 31.44 & 0.949
%         & 34.33 & 0.971
%         & 27.97 & 0.904 \\
%         Voxel (only 3D) & 13.6 M
%         & 32.35 & 0.958
%         & 35.10 & 0.975
%         & 28.35 & 0.912\\
%         Hybrid (2D + 3D) & 13.2 M 
%         & \textbf{32.64} & \textbf{0.959}
%         & \textbf{35.40} & \textbf{0.976}
%         & \textbf{28.44} & \textbf{0.916} \\
%         \bottomrule
%     \end{tabular}
%     }
%     \vspace{+2mm}
%     \caption{Ablation evaluations on the feature grid design. We highlight the best scores in \textbf{bold}.}
%     \label{tab:ablation_grid}
% \end{table}


==> tables/main/ablation_sparsity.tex <==
\begin{table}[!ht]
    \centering
    \resizebox{0.6\textwidth}{!}{
    \begin{tabular}{lrcccc}
    \toprule
    & Train$\downarrow$ & Inference$\uparrow$  & PSNR$\uparrow$ & SSIM$\uparrow$ \\
    \midrule
    Ours-F2 (w/o $\mathcal{L}_{\text{sparsity}}$)
    & 6.4 m & 3.3 fps & 32.69 & 0.959 \\
    Ours-F2 (w/ $\mathcal{L}_{\text{sparsity}}$)
    & 6.1 m & 3.8 fps & 32.64 & 0.959 \\
    \midrule
    Ours-F8 (w/o $\mathcal{L}_{\text{sparsity}}$)
    & 14.7 m & 2.2 fps & 33.60 & 0.964 \\
    Ours-F8 (w/ $\mathcal{L}_{\text{sparsity}}$)
    & 13.9 m & 2.7 fps & 33.59 & 0.964 \\
    \bottomrule
    \end{tabular}
    }
    \vspace{+2mm}
    \caption{Ablation evaluations on the use of sparsity loss. We report train time and inference speed with reconstruction quality (PSNR and SSIM) on Sythetic-NeRF datatset.}
    \label{tab:ablation_sparsity}
\end{table}


==> tables/main/comparison_with_models.tex <==
\begin{table*}[ht]
    \centering
    \caption{
    Quantitative results of model size and reconstruction quality on the Synthetic-NeRF dataset, Synthetic-NSVF dataset, and Tanks \& Temples dataset. We divide the baselines into data-structure-based models and compression-based models. $\dagger$ denotes that we provide scores reported in the original paper. All our models are scaled by the feature dimension $F$; for instance, Ours-F2 denotes a variant with feature dimension $F=2$. We highlight the \colorbox{yellow!75} {best score} and \colorbox{yellow!25}{second-best score}.
    % \jaesik{Comparing with Neus2?}~\seungjoo{I will check that it is reasonable model as a baseline}\jaesik{Size and time for other datasets?}\seungjoo{Such size and time for other datasets are also measured but I did not include it as the length of table could be too large. Is it better to add it? Or chage the size and time for avg values across all datasets?}
    % The first four rows show models with a storage capacity of less than 5 MB, while the rows below show models with a capacity exceeding 5 MB. All our models are scaled by the hash table size. We highlight the \colorbox{yellow!75}{best score} and \colorbox{yellow!25}{second-best score}.
    }
    \resizebox{\textwidth}{!}{
    \begin{tabular}{lccccccccc}
        \toprule
            \multirow{2}{*}{Method} &
            \multicolumn{3}{c}{Synthetic-NeRF} &
            \multicolumn{3}{c}{Synthetic-NSVF} &
            \multicolumn{3}{c}{Tanks \& Temples} \\
            \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}
            & Size (MB)$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ 
            & Size (MB)$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ 
            & Size (MB)$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ \\
        \midrule
        % \multicolumn{9}{c}{Small models} \\
        % \midrule
        DVGO~\cite{sun2022direct,sun2022improved}
        & 655.3 & 31.96 & 0.956 
        & 653.7 & 35.01 & 0.975 
        & 652.8 & 28.36 & 0.911 \\
        Plenoxels~\cite{fridovich2022plenoxels} 
        & 778.2 & 31.72 & 0.958 
        & 803.6 & 34.15 & 0.978 
        & 892.8 & 26.87 & 0.912 \\
        TensoRF-CP~\cite{chen2022tensorf} 
        & 3.9 & 31.66 & 0.950
        & 4.1 & 34.57 & 0.971
        & 4.0 & 27.93 & 0.901 \\
        TensoRF-VM~\cite{chen2022tensorf} 
        & 72.4 & 33.24 & 0.963
        & 71.6 & \cellcolor{yellow!75} 36.73 & \cellcolor{yellow!25} 0.982
        & 72.5 & \cellcolor{yellow!75} 28.65 & 0.922 \\
        CCNeRF-CP~\cite{tang2022compressible}
        & 1.5 & 29.30 & 0.937
        & 1.6 & 31.99 & 0.950
        & 1.6 & 23.53 & 0.862 \\
        CCNeRF-HY~\cite{tang2022compressible}
        & 72.1 & 31.22 & 0.947
        & 71.7 & 34.57 & 0.974
        & 73.7 & 24.76 & 0.886 \\
        Instant-NGP~\cite{muller2022instant}
        & 24.6 & 32.66 & 0.958
        & 24.6 & 33.01 & 0.973
        & 24.5 & 27.72 & \cellcolor{yellow!75} 0.926 \\
        K-Planes-explicit~\cite{fridovich2023k}
        & 384.7 & 32.19 & 0.960
        & 383.9 & 31.20 & 0.952
        & 383.9 & 28.01 & 0.921 \\
        K-Planes-hybrid~\cite{fridovich2023k}
        & 383.9 & 32.31 & 0.961
        & 383.9 & 31.18 & 0.951
        & 384.7 & 28.01 & 0.921 \\
        \midrule
        Re:DVGO-High$^\dagger$~\cite{deng2023compressing}
        & 2.0 & 31.08 & 0.944
        & 2.5 & 34.90 & 0.969
        & 1.6 & 27.90 & 0.894 \\
        Re:Plenoxels-High$^\dagger$~\cite{deng2023compressing}
        & 54.7 & 30.97 & 0.944
        & - & - & -
        & 85.5 & 27.34 & 0.896 \\
        Re:TensoRF-High$^\dagger$~\cite{deng2023compressing}
        & 7.9 & 32.81 & 0.956
        & 8.5 & 36.14 & 0.978
        & 6.7 & 28.24 & 0.907 \\
        VQ-DVGO$^\dagger$~\cite{li2022compressing}
        & \cellcolor{yellow!25} 1.4 & 31.77 & 0.954
        & \cellcolor{yellow!25} 1.3 & 34.72 & 0.974
        & \cellcolor{yellow!25} 1.4 & 28.26 & 0.909 \\
        VQ-Plenoxels$^\dagger$~\cite{li2022compressing}
        & 13.7 & 31.53 & 0.956
        & 11.9 & 33.91 & 0.976
        & 14.3 & 26.73 & 0.908 \\
        VQ-TensoRF$^\dagger$~\cite{li2022compressing}
        & 3.6 & 32.86 & 0.960
        & 4.1 & 36.16 & 0.980
        & 3.3 & 28.20 & 0.913 \\
        \midrule
        Ours-F1
        & \cellcolor{yellow!75} 0.7 & 31.53 & 0.949
        & \cellcolor{yellow!75} 0.8 & 34.26 & 0.971 
        & \cellcolor{yellow!75} 0.8 & 28.02 & 0.906 \\
        Ours-F2
        & \cellcolor{yellow!25} 1.4 & 32.64 & 0.959
        & 1.5 & 35.40 & 0.976
        & 1.5 & 28.44 & 0.916 \\
        Ours-F4
        & 2.8 & \cellcolor{yellow!25} 33.26 & \cellcolor{yellow!25} 0.961
        & 2.9  & 36.17 & 0.983
        & 2.9 & \cellcolor{yellow!25} 28.62 & \cellcolor{yellow!25}0.924 \\
        Ours-F8
        & 5.8 & \cellcolor{yellow!75} 33.59 & \cellcolor{yellow!75} 0.964
        & 5.9 & \cellcolor{yellow!25} 36.61 & \cellcolor{yellow!75} 0.983
        & 5.9 & \cellcolor{yellow!75} 28.65 & \cellcolor{yellow!75} 0.926 \\
        \bottomrule
    \end{tabular}
    }
    \vspace{+2mm}
    \label{tab:comparion_models}
    \vspace{-2mm}
\end{table*}

==> tables/main/comparison_with_models_backup.tex <==
% \begin{table*}[ht]
%     \centering
%     \caption{
%     Quantitative results of reconstruction quality on the Synthetic-NeRF dataset, Synthetic-NSVF dataset, and Tanks \& Temples dataset. We divide the baselines into data-structure-based models and compression-based models. $\dagger$ denotes that we provide scores reported in the original paper. All our models are scaled by the feature dimension $F$; for instance, Ours-F2 denotes a variant with feature dimension $F=2$. We highlight the \colorbox{yellow!75} {best score} and \colorbox{yellow!25}{second-best score}.\jaesik{Comparing with Neus2?}~\seungjoo{I will check that it is reasonable model as a baseline}\jaesik{Size and time for other datasets?}
%     }
%     \resizebox{0.75\textwidth}{!}{
%     \begin{tabular}{lcccccc}
%         \toprule
%             \multirow{2}{*}{Method} &
%             \multicolumn{2}{c}{Synthetic-NeRF} &
%             \multicolumn{2}{c}{Synthetic-NSVF} &
%             \multicolumn{2}{c}{Tanks \& Temples} \\
%             \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
%             & PSNR$\uparrow$ & SSIM$\uparrow$ 
%             & PSNR$\uparrow$ & SSIM$\uparrow$ 
%             & PSNR$\uparrow$ & SSIM$\uparrow$   \\
%         \midrule
%         % \multicolumn{9}{c}{Small models} \\
%         % \midrule
%         DVGO~\cite{sun2022direct,sun2022improved}
%         & 31.96 & 0.956 
%         & 35.01 & 0.975 
%         & 28.36 & 0.911 \\
%         Plenoxels~\cite{fridovich2022plenoxels} 
%         & 31.72 & 0.958 
%         & 34.15 & 0.978 
%         & 26.87 & 0.912 \\
%         TensoRF-CP~\cite{chen2022tensorf} 
%         & 31.66 & 0.950
%         & 34.57 & 0.971
%         & 27.93 & 0.901 \\
%         TensoRF-VM~\cite{chen2022tensorf} 
%         & 33.24 & 0.963
%         & \cellcolor{yellow!75} 36.73 & \cellcolor{yellow!25} 0.982
%         & \cellcolor{yellow!75} 28.65 & 0.922 \\
%         CCNeRF-CP~\cite{tang2022compressible}
%         & 29.30 & 0.937
%         & 31.99 & 0.950
%         & 23.53 & 0.862 \\
%         CCNeRF-HY~\cite{tang2022compressible}
%         & 31.22 & 0.947
%         & 34.57 & 0.974
%         & 24.76 & 0.886 \\
%         Instant-NGP~\cite{muller2022instant}
%         & 32.66 & 0.958
%         & 33.01 & 0.973
%         & 27.72 & \cellcolor{yellow!75} 0.926 \\
%         K-Planes-explicit~\cite{fridovich2023k}
%         & 32.19 & 0.960
%         & 31.20 & 0.952
%         & 28.01 & 0.921 \\
%         K-Planes-hybrid~\cite{fridovich2023k}
%         & 32.31 & 0.961
%         & 31.18 & 0.951
%         & 28.01 & 0.921 \\
%         \midrule
%         Re:DVGO-High$\dagger$~\cite{deng2023compressing}
%         & 31.08 & 0.944
%         & 34.90 & 0.969
%         & 27.90 & 0.894 \\
%         Re:Plenoxels-High$\dagger$~\cite{deng2023compressing}
%         & 30.97 & 0.944
%         & - & -
%         & 27.34 & 0.896 \\
%         Re:TensoRF-High$\dagger$~\cite{deng2023compressing}
%         & 32.81 & 0.956
%         & 36.14 & 0.978
%         & 28.24 & 0.907 \\
%         VQ-DVGO$\dagger$~\cite{li2022compressing}
%         & 31.77 & 0.954
%         & 34.72 & 0.974
%         & 28.26 & 0.909 \\
%         VQ-Plenoxels$\dagger$~\cite{li2022compressing}
%         & 31.53 & 0.956
%         & 33.91 & 0.976
%         & 26.73 & 0.908 \\
%         VQ-TensoRF$\dagger$~\cite{li2022compressing}
%         & 32.86 & 0.960
%         & 36.16 & 0.980
%         & 28.20 & 0.913 \\
%         \midrule
%         Ours-F1
%         & 31.53 & 0.949
%         & 34.26 & 0.971 
%         & 28.02 & 0.906 \\
%         Ours-F2
%         & 32.64 & 0.959
%         & 35.40 & 0.976
%         & 28.44 & 0.916 \\
%         Ours-F4
%         & \cellcolor{yellow!25} 33.26 & \cellcolor{yellow!25} 0.961
%         & 36.17 & 0.983
%         & \cellcolor{yellow!25} 28.62 & \cellcolor{yellow!25}0.924 \\
%         Ours-F8
%         & \cellcolor{yellow!75} 33.59 & \cellcolor{yellow!75} 0.964
%         & \cellcolor{yellow!25} 36.61 & \cellcolor{yellow!75} 0.983
%         & \cellcolor{yellow!75} 28.65 & \cellcolor{yellow!75} 0.926 \\
%         \bottomrule
%     \end{tabular}
%     }
%     \vspace{+2mm}
%     \label{tab:comparion_models}
%     \vspace{-2mm}
% \end{table*}


\begin{table*}[ht]
    \centering
    \caption{
    Quantitative results of model size and reconstruction quality on the Synthetic-NeRF dataset, Synthetic-NSVF dataset, and Tanks \& Temples dataset. We divide the baselines into data-structure-based models and compression-based models. $\dagger$ denotes that we provide scores reported in the original paper. All our models are scaled by the feature dimension $F$; for instance, Ours-F2 denotes a variant with feature dimension $F=2$. We highlight the \colorbox{yellow!75} {best score} and \colorbox{yellow!25}{second-best score}.
    % \jaesik{Comparing with Neus2?}~\seungjoo{I will check that it is reasonable model as a baseline}\jaesik{Size and time for other datasets?}\seungjoo{Such size and time for other datasets are also measured but I did not include it as the length of table could be too large. Is it better to add it? Or chage the size and time for avg values across all datasets?}
    % The first four rows show models with a storage capacity of less than 5 MB, while the rows below show models with a capacity exceeding 5 MB. All our models are scaled by the hash table size. We highlight the \colorbox{yellow!75}{best score} and \colorbox{yellow!25}{second-best score}.
    }
    \resizebox{0.9\textwidth}{!}{
    \begin{tabular}{lccccccc}
        \toprule
            \multirow{2}{*}{Method} &
            \multicolumn{3}{c}{Synthetic-NeRF} &
            \multicolumn{2}{c}{Synthetic-NSVF} &
            \multicolumn{2}{c}{Tanks \& Temples} \\
            \cmidrule(lr){2-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8}
            & Size (MB)$\downarrow$
            & PSNR$\uparrow$ & SSIM$\uparrow$ 
            & PSNR$\uparrow$ & SSIM$\uparrow$ 
            & PSNR$\uparrow$ & SSIM$\uparrow$   \\
        \midrule
        % \multicolumn{9}{c}{Small models} \\
        % \midrule
        DVGO~\cite{sun2022direct,sun2022improved}
        & 655.3
        & 31.96 & 0.956 
        & 35.01 & 0.975 
        & 28.36 & 0.911 \\
        Plenoxels~\cite{fridovich2022plenoxels} 
        & 778.2
        & 31.72 & 0.958 
        & 34.15 & 0.978 
        & 26.87 & 0.912 \\
        TensoRF-CP~\cite{chen2022tensorf} 
        & 3.9
        & 31.66 & 0.950
        & 34.57 & 0.971
        & 27.93 & 0.901 \\
        TensoRF-VM~\cite{chen2022tensorf} 
        & 72.4
        & 33.24 & 0.963
        & \cellcolor{yellow!75} 36.73 & \cellcolor{yellow!25} 0.982
        & \cellcolor{yellow!75} 28.65 & 0.922 \\
        CCNeRF-CP~\cite{tang2022compressible}
        & 1.5
        & 29.30 & 0.937
        & 31.99 & 0.950
        & 23.53 & 0.862 \\
        CCNeRF-HY~\cite{tang2022compressible}
        & 72.1
        & 31.22 & 0.947
        & 34.57 & 0.974
        & 24.76 & 0.886 \\
        Instant-NGP~\cite{muller2022instant}
        & 24.6
        & 32.66 & 0.958
        & 33.01 & 0.973
        & 27.72 & \cellcolor{yellow!75} 0.926 \\
        K-Planes-explicit~\cite{fridovich2023k}
        & 384.7
        & 32.19 & 0.960
        & 31.20 & 0.952
        & 28.01 & 0.921 \\
        K-Planes-hybrid~\cite{fridovich2023k}
        & 383.9
        & 32.31 & 0.961
        & 31.18 & 0.951
        & 28.01 & 0.921 \\
        \midrule
        Re:DVGO-High$\dagger$~\cite{deng2023compressing}
        & 2.0
        & 31.08 & 0.944
        & 34.90 & 0.969
        & 27.90 & 0.894 \\
        Re:Plenoxels-High$\dagger$~\cite{deng2023compressing}
        & 54.7
        & 30.97 & 0.944
        & - & -
        & 27.34 & 0.896 \\
        Re:TensoRF-High$\dagger$~\cite{deng2023compressing}
        & 7.9
        & 32.81 & 0.956
        & 36.14 & 0.978
        & 28.24 & 0.907 \\
        VQ-DVGO$\dagger$~\cite{li2022compressing}
        & \cellcolor{yellow!25} 1.4
        & 31.77 & 0.954
        & 34.72 & 0.974
        & 28.26 & 0.909 \\
        VQ-Plenoxels$\dagger$~\cite{li2022compressing}
        & 13.7
        & 31.53 & 0.956
        & 33.91 & 0.976
        & 26.73 & 0.908 \\
        VQ-TensoRF$\dagger$~\cite{li2022compressing}
        & 3.6
        & 32.86 & 0.960
        & 36.16 & 0.980
        & 28.20 & 0.913 \\
        \midrule
        Ours-F1
        & \cellcolor{yellow!75} 0.7
        & 31.53 & 0.949
        & 34.26 & 0.971 
        & 28.02 & 0.906 \\
        Ours-F2
        & \cellcolor{yellow!25} 1.4
        & 32.64 & 0.959
        & 35.40 & 0.976
        & 28.44 & 0.916 \\
        Ours-F4
        & 2.8
        & \cellcolor{yellow!25} 33.26 & \cellcolor{yellow!25} 0.961
        & 36.17 & 0.983
        & \cellcolor{yellow!25} 28.62 & \cellcolor{yellow!25}0.924 \\
        Ours-F8
        & 5.8
        & \cellcolor{yellow!75} 33.59 & \cellcolor{yellow!75} 0.964
        & \cellcolor{yellow!25} 36.61 & \cellcolor{yellow!75} 0.983
        & \cellcolor{yellow!75} 28.65 & \cellcolor{yellow!75} 0.926 \\
        \bottomrule
    \end{tabular}
    }
    \vspace{+2mm}
    \label{tab:comparion_models}
    \vspace{-2mm}
\end{table*}

==> tables/main/model_setting.tex <==
\begin{table}[!ht]
    \centering
    \begin{tabular}{lccc}
    \toprule
     & $T_{\text{2D}}$ & $T_{\text{3D}}$ & \# of params\\
    \midrule
    Ours-S & $2^{15}$ & $2^{17}$ & 3.9 M $\times F$  \\ 
    Ours-B & $2^{17}$ & $2^{19}$ & 13.2 M $\times F$ \\ 
    \bottomrule
    \end{tabular}
    \vspace{+2mm}
    \caption{Details of feature grid variants.\jaesik{Prepare ablation study when using 2D grid or 3D grid only}}
    \label{tab:model_setting}
\end{table}

